Distance-Based Propagation for Efficient Knowledge Graph Reasoning

Knowledge graph completion (KGC) aims to predict unseen edges in knowledge graphs (KGs), resulting in the discovery of new facts. A new class of methods have been proposed to tackle this problem by aggregating path information. These methods have shown tremendous ability in the task of KGC. However they are plagued by efficiency issues. Though there are a few recent attempts to address this through learnable path pruning, they often sacrifice the performance to gain efficiency. In this work, we identify two intrinsic limitations of these methods that affect the efficiency and representation quality. To address the limitations, we introduce a new method, TAGNet, which is able to efficiently propagate information. This is achieved by only aggregating paths in a fixed window for each source-target pair. We demonstrate that the complexity of TAGNet is independent of the number of layers. Extensive experiments demonstrate that TAGNet can cut down on the number of propagated messages by as much as 90% while achieving competitive performance on multiple KG datasets. The code is available at https://github.com/HarryShomer/TAGNet.

==> sections/motivation.tex <==
\section{Limitations of Current Methods} \label{sec:limitations}
% A main 
Inefficiency is a core problem of path-based GNNs such as NBFNet~\cite{nbfnet} and RED-GNN~\cite{redgnn}, which severely limits their adoptions in real-world applications. \ym{Probably, we do not even mention this$\rightarrow$ Due to their inefficiency, path-based GNN models typically only propagate for a small number of layers, which limits their capability for learning representations for distant nodes. } 

% To improve the efficiency, 
% As such, recent methods  $\text{A}^*\text{Net}$ and AdaProp learn to prune paths to propagate more efficiently. However they too suffer from several limitations. In the following, we will detail the limitations of current methods which inspire our proposed method in Section~\ref{sec:framework}. 

% Due to their inefficiency, current path-based GNNs are unable to propagate deeply. This poses a severe problem in learning quality representations for nodes far from the source node. We refer to such nodes as \textit{distant nodes}. A path-based GNN with $T$ layers can only learn representations for nodes within $T$ hops of the source node. Therefore, in order to learn a representation for a node $v$ where $\text{dist}(s, v)> T$, the number of layers needs to be increased accordingly. However, the time complexity of all existing methods is proportional to the number of layers. This makes it impossible to learn representations for distant nodes without significantly sacrificing efficiency. 

% Furthermore, even if a distant node $v$ can be reached, it is likely that little path information will be aggregated. For example when $T=6$ and $\text{dist}(s, v) = 6$, we only aggregate paths of length $6$ for the node $v$. This lack of aggregated path information strongly limits the power of node $v$'s representation.
To improve the efficiency, several recent works have been proposed including $\text{A}^*\text{Net}$~\cite{ANet} and AdaProp~\cite{Adaprop}. These methods aim at reducing the number of messages being passed by only propagating to a subset of nodes at each iteration. They typically learn a parameterized model to select this set of nodes in a data-driven way without strict principles, which leads to the following limitations. 
% The inability to propagate deeply has inspired recent works that propose to learn which paths to propagate to. Two such frameworks, $\text{A}^*\text{Net}$~\cite{ANet} and AdaProp~\cite{Adaprop}, only propagate to a subset of the available nodes at each iteration. The subset of nodes to propagate to is determined via a set of learnable parameters. However, there are several disadvantages with such approaches:
\begin{enumerate}
    \item \textbf{Unknown path importance}: There is no ground truth for path importance. This makes it impossible to determine whether the model is selecting the correct paths to prune or not. Since there is no supervision, it is difficult to learn the model for pruning. 
    \item \textbf{Cost of learnable pruning}: Learning how to prune negates some of the efficiency gains made by pruning. For example, $\text{A}^*\text{Net}$ determines which nodes to propagate at iteration $t$ by applying a priority function to all nodes $v \in V$ and choosing the top $K$ nodes. This adds a significant cost of $T \lvert V \rvert d^2$ to the complexity. Furthermore, the complexity of $\text{A}^*\text{Net}$ and AdaProp are still proportional to the number of layers, severely compromising their ability to propagate deeper. 
    \item \textbf{Lack of understanding}: Since the pruning is done via learnable parameters, the pruning strategy can be considered a black box. This makes it difficult to understand why the model chooses some paths over others.
    \item \textbf{Sacrificed Performance}: Both $\text{A}^*\text{Net}$ and AdaProp struggle to perform well in both transductive and inductive settings, which further indicates the learned pruning strategies are not optimal. More discussion and results are presented in Section~\ref{XXX.} \ym{To be updated..}
    % as shown in Table~\ref{tab:transductive} and Table~\ref{tab:inductive}.  
\end{enumerate}
This set of issues motivates us to design a new path-pruning method that doesn't suffer from any of the aforementioned issues. 

% More succinctly, we can distill the set of problems down into two main motivations when designing our new framework:
% \begin{enumerate}
%     \item \textit{Design a pruning strategy that is both efficient a.} 
%     \item \textit{Design a path-based GNN where the number of layers is decoupled from the complexity, allowing for deeper propagation.}
% \end{enumerate}
% In the following section we present our method that addresses both of our motivations.
% The \textbf{first} limitation is the limited ability of propagating deeply and learning representations of distant nodes. This is a result of the complexity of all existing path-based GNNs being proportional to the number of layers. The \textbf{second} limitation concerns the inherit difficulties of learnable path-pruning. In the following, we will detail each limitation which inspires us with a specific motivation to design our proposed method in Section~\ref{sec:framework}. 
% \newline\newline 
% \noindent \underline{\textbf{Limitation \#1: Inability to Propagate Deeply}}
% \newline\newline
% Due to their inefficiency, current path-based GNNs are unable to propagate deeply. This poses a severe problem of learning quality representations for nodes far from the source node. We refer to such nodes as \textit{distant nodes}. Path-based GNNs with $T$ layers can only learn representations for nodes within \jt{should be $T$ here?} hops of the source node. Therefore, in order to learn a representation for a node $v$ where $\text{dist}(s, v)> T$, the number of layers needs to be increased accordingly. However, the time complexity of all existing methods is proportional to the number of layers. This makes it impossible to learn representations for distant nodes without significantly sacrificing efficiency. 
 
% Furthermore, even if a distant node $v$ can be reached ($\text{dist}(s, v) \leq T$), it is likely that very little path information will be aggregated. For example when $T=6$ and $\text{dist}(s, v) = 6$, we only aggregate paths of length $6$ for the node $v$. Therefore, the inefficiency problem also limits the aggregation capabilities of distant nodes. This lack of aggregated path information strongly limits the power of node $v$'s representation.
% \newline\newline
% \noindent \underline{Motivation \#1:} \textit{Design a path-based GNN where the number of layers is decoupled from the complexity, allowing for deeper propagation.}
% \newline\newline
% \noindent \underline{\textbf{Limitation \#2: Difficulties of Learnable Path-Pruning}}
% \newline\newline
% The previous limitation has inspired recent works that propose to learn which paths to consider. Two such frameworks, $\text{A}^*\text{Net}$ and AdaProp, only propagate to a subset of the available nodes at each iteration. The subset of nodes to propagate to is determined via a set of learnable parameters. However, there are several disadvantages with such approaches:\begin{enumerate}
%     \item \textbf{Unknown path importance}: There is no ground truth for path importance. This makes it impossible to determine whether the model is selecting the correct paths to prune or not. Since there is no supervision, it is a difficult problem to optimize.
%     \item \textbf{Cost of learnable pruning}: Learning how to prune negates some of the efficiency gains made by pruning. For example, $\text{A}^*\text{Net}$ determines which nodes to propagate at iteration $t$ by applying a priority function to all nodes $v \in V$ and choosing the top $K$ nodes. This adds a significant cost of $T \lvert V \rvert d^2$ to the complexity.
%     \item \textbf{Lack of understanding}: Since the pruning is done via learnable parameters, the pruning strategy can be considered a black box. This makes it difficult to understand why the model chooses some paths over others.
%     \item \textbf{Sacrificed Performance}: Both $\text{A}^*\text{Net}$ and AdaProp struggle to perform well in both transductive and inductive settings as shown in Table~\ref{tab:transductive} and Table~\ref{tab:inductive}.  
% \end{enumerate}

% \noindent \underline{Motivation \#2:} \textit{Design a pruning strategy that is efficient and understandable.}
% \newline\newline
% \noindent In the following section we present our method that addresses both of our motivations.


% \subsection{Non-Informative Messages} \label{sec:non_informative}

% Path-based GNNs work by diffusing information from the source node to all other nodes over $T$ iterations. Due to this, at iteration $t$ a node $v$ may have not have aggregated any information yet. We give an example from Figure~\ref{fig:prop-example}. At iteration 1, node $6$ hasn't aggregated any path information yet as it's a 2-hop neighbor of the source. Therefore by aggregating node $6$ at iteration $1$ no additional path information is aggregated. Both $\text{A}^{*}Net$ and NBFNet aggregate such messages (to our knowledge AdaProp and RED-GNN do not).

% We refer to any message that contains such nodes as \textit{non-informative messages}. Since these additional messages add to the overall complexity and contain no path information we wish to avoid aggregating them. \harry{The following can probably be said better} However, just because they contain no path information doesn't mean they can't still be useful. Even though in practice all target nodes are initialized to zero, due to biases in the linear projections and layer normalization layers the nodes involved in non-informative messages typically accumulate some values over time. As such, there may still be some value in aggregating non-informative messages as they can inform a node of its surrounding neighborhood. We explore this idea further in Section~\ref{}.
% \newline\newline
% \noindent \underline{Motivation \#3:} \textit{Avoid explicitly aggregating non-informative messages to improve efficiency}.

 



